The Delayed Stabilizer ZX-Calculus

Many stabilizer quantum error-correcting codes are built from a finite pattern repeated across space or time, such as lattice codes, translation-invariant graph states, and quantum convolutional codes. Ordinary stabilizer ZX-diagrams capture only finite truncations of such systems, obscuring the repeated structure that defines them. We introduce the delayed stabilizer ZX-calculus, a finite graphical language for these infinite, translation-invariant processes. It extends the odd-prime-dimensional stabilizer ZX-calculus with a single new generator, the delay, which feeds data from one time step to the next. We equip the calculus with two semantics. In the first semantics, we interpret the behaviour of a delayed ZX-diagram as an equivalence class of sequences of quantum channels; where two sequences are identified if they have the same information content. We show that the behaviour of a delayed ZX-diagram uniquely determines an infinite stabilizer group. In the second semantics, we interpret the delay as a formal variable, encoding the translation-invariant families of Pauli operators as generating functions. This allows us to represent a delayed ZX-diagram in terms of a tableau of generating functions, from which the infinite stabilizer group can be recovered. Finally, we give a complete axiomatization of the delayed stabilizer ZX-calculus, featuring generalised Euler decomposition and colour change rules. Using generalised forms of local complementation and pivoting, we reduce every diagram to a unique normal form. This establishes soundness, universality, and completeness for the generating tableau semantics.

==> style/tikz/bubbles.tex <==

\newcommand{\wbubbleTailEdgeInset}{8pt} %
\newcommand{\wbubbleTailWidthFrac}{0.65} %
\newcommand{\wbubbleTailMinWidth}{2pt}
\newcommand{\wbubbleTailMaxWidth}{13pt}  %
\newcommand{\wbubbleTailHeightFrac}{0.55}%
\newcommand{\wbubbleTailMinHeight}{2pt}
\newcommand{\wbubbleTailMaxHeight}{8pt}  %

\newcommand{\wbubbleShiftWest}{0pt} %
\newcommand{\wbubbleShiftEast}{\wbubbleShiftWest}
\newcommand{\wbubbleThinSpiderTipRadius}{2.35mm}
\newcommand{\wbubbleThickSpiderTipRadius}{2.7mm}
\newcommand{\wbubbleSpiderTipRadius}{\wbubbleThinSpiderTipRadius}
\newcommand{\registerwbubbletipradius}[1]{%
  \expandafter\xdef\csname wbubbletipradius:\tikzlastnode\endcsname{#1}%
}
\newcommand{\setwbubbletipradius}{%
  \ifcsname wbubbletipradius:\tikztotarget\endcsname
    \edef\wbubbleSpiderTipRadius{\csname wbubbletipradius:\tikztotarget\endcsname}%
  \else
    \edef\wbubbleSpiderTipRadius{\wbubbleThinSpiderTipRadius}%
  \fi
}
\tikzstyle{phase-thin-spider}=[append after command={\pgfextra{\registerwbubbletipradius{\wbubbleThinSpiderTipRadius}}}]
\tikzstyle{phase-thick-spider}=[append after command={\pgfextra{\registerwbubbletipradius{\wbubbleThickSpiderTipRadius}}}]
\newcommand{\wbubbleCtrl}{2pt} %
\newcommand{\wbubbleOverlap}{0pt}
\newcommand{\wbubbleTipSpread}{12}
\newcommand{\wbubbleTipCtrl}{3pt}
\newcommand{\wbubbleBaseBow}{0pt}
\newcommand{\bubbleWhiteBaseBow}{0pt}
\newcommand{\bubbleBlackBaseBow}{0pt}
\tikzstyle{use-bow-white}=[/utils/exec=\def\wbubbleBaseBow{\bubbleWhiteBaseBow}]
\tikzstyle{use-bow-black}=[/utils/exec=\def\wbubbleBaseBow{\bubbleBlackBaseBow}]

\newcommand{\phaseShadowXShift}{2pt}
\newcommand{\phaseShadowYShift}{-2pt}
\newcommand{\phaseShadowOpacity}{.20}
\colorlet{addspiderphaseshadowcolor}{black!70!addspiderphasefillcolor}
\colorlet{copyspiderphaseshadowcolor}{black!70!copyspiderphasefillcolor}
\newcommand{\phaseShadowColor}{black}
\tikzstyle{bubble-skin}=[on layer=frontlayer, overlay]
\tikzstyle{bubble-layer-node}=[node on layer=frontlayer]

\tikzstyle{bubble-white-node}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{addspiderphaseshadowcolor}, draw=none, text=addspiderphasetextcolor, text opacity=1]
\tikzstyle{bubble-black-node}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{copyspiderphaseshadowcolor}, draw=none, text=copyspiderphasetextcolor, text opacity=1]
\tikzstyle{bubble-white-node-solo}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{addspiderphaseshadowcolor}, fill=addspiderphasefillcolor, draw=none, text=addspiderphasetextcolor, fill opacity=.85, text opacity=1]
\tikzstyle{bubble-black-node-solo}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{copyspiderphaseshadowcolor}, fill=copyspiderphasefillcolor, draw=none, text=copyspiderphasetextcolor, fill opacity=.9, text opacity=1]
\tikzstyle{bubble-white-path}=[on layer=labeltextlayer, overlay, fill=addspiderphasefillcolor, fill opacity=.85]
\tikzstyle{bubble-black-path}=[on layer=labeltextlayer, overlay, fill=copyspiderphasefillcolor, fill opacity=.9]
\newcommand{\bubbleCornerRadius}{4pt} %
\newcommand{\bubbleMinimumDimension}{12pt} %
\newcommand{\phasebubbleshadow}{%
  \begin{pgfonlayer}{phaseshadowlayer}%
    \path[
      overlay,
      draw=none,
      fill=\phaseShadowColor,
      fill opacity=\phaseShadowOpacity,
      rounded corners=\bubbleCornerRadius
    ]
      ($(\tikzlastnode.south west)+(\phaseShadowXShift,\phaseShadowYShift)$)
      rectangle
      ($(\tikzlastnode.north east)+(\phaseShadowXShift,\phaseShadowYShift)$);
  \end{pgfonlayer}%
  % The bubble body/shadow is drawn with `overlay`, on purpose, so it never
  % perturbs picture layout in normal compiles. But that also means tikz
  % externalization -- which crops each picture to its computed bounding box
  % -- would clip it off. So, only while actually rendering the external
  % image, register its true extent (via a paint-free path) so the crop
  % includes it.
  \tikzifexternalizing{%
    \path[draw=none,fill=none]
      ($(\tikzlastnode.south west)+(\phaseShadowXShift,\phaseShadowYShift)$)
      rectangle
      ($(\tikzlastnode.north east)+(\phaseShadowXShift,\phaseShadowYShift)$);
  }{}%
}
\tikzstyle{bubble-base}=[
  rectangle, rounded corners=\bubbleCornerRadius, ultra thin,
  inner xsep=2pt, inner ysep=0.5pt, %
  minimum height=\bubbleMinimumDimension,
  minimum width=\bubbleMinimumDimension,
  font={\scriptsize\boldmath}, node on layer=frontlayer,
  append after command={\pgfextra{%
    \phasebubbleshadow
    \tikzifexternalizing{%
      \path[draw=none,fill=none] (\tikzlastnode.south west) rectangle (\tikzlastnode.north east);
    }{}%
  }}
]

\tikzstyle{wphase}=[bubble-base, bubble-white-node, tikzit category=ZX, tikzit fill=white, tikzit draw=white]
\tikzstyle{bphase}=[bubble-base, bubble-black-node, tikzit category=ZX, tikzit fill=black, tikzit draw=white]
\tikzstyle{wphasesolo}=[bubble-base, bubble-white-node-solo, tikzit category=ZX, tikzit fill=white, tikzit draw=white]
\tikzstyle{bphasesolo}=[bubble-base, bubble-black-node-solo, tikzit category=ZX, tikzit fill=black, tikzit draw=white]

\tikzstyle{bubble-tail}=[bubble-white-path] %

\newcommand{\bubblerect}{%
  [rounded corners=\bubbleCornerRadius]
  (\tikztostart.south west) rectangle (\tikztostart.north east)
  [sharp corners]%
}

\newcommand{\bubblefill}[1]{%
  \path[bubble-tail] \bubblerect #1;
  % \bubblerect and #1 (the pointer tail) are drawn on an `overlay` path, on
  % purpose -- see the note in \phasebubbleshadow. Register their true extent
  % into the picture's bounding box only when generating the external image.
  \tikzifexternalizing{%
    \path[draw=none,fill=none] \bubblerect #1;
  }{}%
}

\makeatletter
\newcommand{\setbubbletailwidth}{%
  \pgfpointdiff{\pgfpointanchor{\tikztostart}{west}}{\pgfpointanchor{\tikztostart}{east}}%
  \edef\bubblenodedim{\the\pgf@x}%
  \pgfmathsetlengthmacro\WB{min(\wbubbleTailMaxWidth,%
        max(\wbubbleTailMinWidth,%
            \wbubbleTailWidthFrac*max(0pt, \bubblenodedim-\wbubbleTailEdgeInset)))}%
}
\newcommand{\setbubbletailheight}{%
  \pgfpointdiff{\pgfpointanchor{\tikztostart}{south}}{\pgfpointanchor{\tikztostart}{north}}%
  \edef\bubblenodedim{\the\pgf@y}%
  \pgfmathsetlengthmacro\WB{min(\wbubbleTailMaxHeight,%
        max(\wbubbleTailMinHeight,%
            \wbubbleTailHeightFrac*max(0pt, \bubblenodedim-\wbubbleTailEdgeInset)))}%
}
\makeatother

\tikzstyle{phasetosouth}=[
  draw=none,
  to path={
    \pgfextra{%
      \setbubbletailwidth
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}{\pgfpointanchor{\tikztostart}{south}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wL)   at ($(\tikztostart.south)+(-.5*\WB, \wbubbleOverlap)$);
      \coordinate (wR)   at ($(\tikztostart.south)+(.5*\WB,  \wbubbleOverlap)$);
      \coordinate (wTip) at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (cL) at ($ (wTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (cR) at ($ (wTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \bubblefill{
        (wL)
          .. controls ($(wL)+(\wbubbleCtrl,0)$) and (cL) .. (wTip)
          .. controls (cR) and ($(wR)+(-\wbubbleCtrl,0)$) .. (wR)
          .. controls ($(wR)+(0,\wbubbleBaseBow)$) and ($(wL)+(0,\wbubbleBaseBow)$) .. (wL)
        -- cycle
      }
    }%
    (\tikztostart) -- (\tikztotarget) \tikztonodes
  }
]

\tikzstyle{phasetonorth}=[draw=none,
  to path={
    \pgfextra{%
      \setbubbletailwidth
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}
                                 {\pgfpointanchor{\tikztostart}{north}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wL)   at ($(\tikztostart.north)+(-.5*\WB,-\wbubbleOverlap)$);
      \coordinate (wR)   at ($(\tikztostart.north)+(.5*\WB, -\wbubbleOverlap)$);
      \coordinate (wTip) at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (cL) at ($ (wTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (cR) at ($ (wTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \bubblefill{
        (wL)
          .. controls ($(wL)+(\wbubbleCtrl,0)$)      and (cL) .. (wTip)
          .. controls (cR) and ($(wR)+(-\wbubbleCtrl,0)$) .. (wR)
          .. controls ($(wR)+(0,-\wbubbleBaseBow)$)  and ($(wL)+(0,-\wbubbleBaseBow)$) .. (wL)
        -- cycle
      }
    }%
    (\tikztostart)--(\tikztotarget)\tikztonodes
  }
]

\tikzstyle{phasetowest}=[draw=none,
  to path={
    \pgfextra{%
      \setbubbletailheight
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}
                                 {\pgfpointanchor{\tikztostart}{west}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wBase) at ($(\tikztostart.west)!\wbubbleOverlap!(\tikztostart.center)$);
      \coordinate (wT)    at ($(wBase)+(0,.5*\WB)$);
      \coordinate (wB)    at ($(wBase)+(0,-.5*\WB)$);
      \coordinate (wTip)  at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (sT)    at ($(wT)+(\wbubbleShiftWest,0)$);
      \coordinate (sB)    at ($(wB)+(\wbubbleShiftWest,0)$);
      \coordinate (sTip)  at ($(wTip)+(\wbubbleShiftWest,0)$);
      \coordinate (sCT) at ($ (sTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (sCB) at ($ (sTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \bubblefill{
        (sT)
          .. controls ($(sT)+(0,-\wbubbleCtrl)$) and (sCT) .. (sTip)
          .. controls (sCB) and ($(sB)+(0,\wbubbleCtrl)$) .. (sB)
          .. controls ($(sB)+(\wbubbleBaseBow,0)$) and ($(sT)+(\wbubbleBaseBow,0)$) .. (sT)
        -- cycle
      }
    }%
    (\tikztostart)--(\tikztotarget)\tikztonodes
  }
]

\tikzstyle{phasetoeast}=[draw=none,
  to path={
    \pgfextra{%
      \setbubbletailheight
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}
                                 {\pgfpointanchor{\tikztostart}{east}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wBase) at ($(\tikztostart.east)!\wbubbleOverlap!(\tikztostart.center)$);
      \coordinate (wT)    at ($(wBase)+(0,.5*\WB)$);
      \coordinate (wB)    at ($(wBase)+(0,-.5*\WB)$);
      \coordinate (wTip)  at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (sT)    at ($(wT)-(\wbubbleShiftWest,0)$);
      \coordinate (sB)    at ($(wB)-(\wbubbleShiftWest,0)$);
      \coordinate (sTip)  at ($(wTip)-(\wbubbleShiftWest,0)$);
      \coordinate (sCT) at ($ (sTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (sCB) at ($ (sTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \bubblefill{
        (sT)
          .. controls ($(sT)+(0,-\wbubbleCtrl)$) and (sCT) .. (sTip)
          .. controls (sCB) and ($(sB)+(0,\wbubbleCtrl)$) .. (sB)
          .. controls ($(sB)+(-\wbubbleBaseBow,0)$) and ($(sT)+(-\wbubbleBaseBow,0)$) .. (sT)
        -- cycle
      }
    }%
    (\tikztostart)--(\tikztotarget)\tikztonodes
  }
]

\tikzstyle{pointer-white}=[-, use-bow-white,
  bubble-tail/.style=bubble-white-path]

\tikzstyle{pointer-black}=[-, use-bow-black,
  bubble-tail/.style=bubble-black-path]


==> style/tikz/hbox.tex <==
\newcommand{\hadCapRadius}{4pt}
\newcommand{\hadLineWidth}{.5pt}
\newcommand{\hadInset}{.4pt}
\newcommand{\hadThickLineWidth}{1.2pt}
\newcommand{\hadThickInset}{0.8pt}
\newcommand{\hadHeadPad}{3pt}
\newcommand{\hadThickHeadPad}{4pt}
\tikzstyle{hadshape}=[shape=rectangle, draw=none, fill=none, text=hadamardtextcolor, minimum height=5pt, minimum width=5pt, inner sep=2pt, font={\scriptsize\boldmath}, anchor=center, outer sep=-\hadInset]
\newcommand{\hadcapnorth}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x2,\y1)+(-\hadInset,\hadInset)$) -- ($(\x1,\y1)+(\hadInset,\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x1,\y2)+(\hadInset,-\hadInset)$) -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) [sharp corners] -- cycle;}
\newcommand{\hadcapsouth}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x1,\y2)+(\hadInset,-\hadInset)$) -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x2,\y1)+(-\hadInset,\hadInset)$) -- ($(\x1,\y1)+(\hadInset,\hadInset)$) [sharp corners] -- cycle;}
\newcommand{\hadcapeast}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x1,\y1)+(\hadInset,\hadInset)$) -- ($(\x1,\y2)+(\hadInset,-\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) -- ($(\x2,\y1)+(-\hadInset,\hadInset)$) [sharp corners] -- cycle;}
\newcommand{\hadcapwest}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x2,\y1)+(-\hadInset,\hadInset)$) -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x1,\y2)+(\hadInset,-\hadInset)$) -- ($(\x1,\y1)+(\hadInset,\hadInset)$) [sharp corners] -- cycle;}


==> style/tikz/multipliers.tex <==

\tikzstyle{mat}=[shape=signal,  fill={multiplierfillcolor}, draw=black, minimum height=6pt, inner sep=1pt, font={\scriptsize\boldmath}, anchor=center, outer sep=-.1cm, signal pointer angle={\arrowangle}, scale={\arrowscaling}]
\newcommand{\matHeadPad}{2.5pt}

\newif\iffastcompile

\makeatletter
\newdimen\@vertangledim
\def\pgf@sh@signal@adaptive@str{adaptive}
\def\pgf@sh@signal@adaptiveh@str{adaptive-h}
\def\pgf@sh@signal@setadaptiveangle{%
  \@vertangledim=\wd\pgfnodeparttextbox
  \edef\@vertangle@wpt{\strip@pt\@vertangledim}%
  \pgfmathparse{min(166.0, max(\arrowangle, \arrowangle + max(0.0, \@vertangle@wpt - 5.0) * 1))}%
  \pgfkeyssetvalue{/pgf/signal pointer angle}{\pgfmathresult}%
}%
\def\pgf@sh@signal@setadaptiveangleh{%
  \@vertangledim=\ht\pgfnodeparttextbox
  \advance\@vertangledim\dp\pgfnodeparttextbox
  \edef\@vertangle@wpt{\strip@pt\@vertangledim}%
  \pgfmathparse{min(166.0, max(\arrowangle, \arrowangle + max(0.0, \@vertangle@wpt - 5.0) * 1))}%
  \pgfkeyssetvalue{/pgf/signal pointer angle}{\pgfmathresult}%
}%
\global\let\pgf@sh@s@signal@orig=\pgf@sh@s@signal
\gdef\pgf@sh@s@signal{%
  \expandafter\ifx\csname pgfk@/pgf/signal pointer angle\endcsname\pgf@sh@signal@adaptive@str
    \iffastcompile
      \pgfkeyssetvalue{/pgf/signal pointer angle}{\arrowangle}%
    \else
      \pgf@sh@signal@setadaptiveangle
    \fi
  \else
    \expandafter\ifx\csname pgfk@/pgf/signal pointer angle\endcsname\pgf@sh@signal@adaptiveh@str
      \iffastcompile
        \pgfkeyssetvalue{/pgf/signal pointer angle}{\arrowangle}%
      \else
        \pgf@sh@signal@setadaptiveangleh
      \fi
    \fi
  \fi
  \pgf@sh@s@signal@orig
}%
\tikzset{adapt-vertical-angle/.style={signal pointer angle=adaptive}}
\tikzset{adapt-horizontal-angle/.style={signal pointer angle=adaptive-h}}
\makeatother

